PoseKernelLifter: Metric Lifting of 3D Human Pose using Sound

Reconstructing the 3D pose of a person in metric scale from a single view image is a geometrically ill-posed problem. For example, we can not measure the exact distance of a person to the camera from a single view image without additional scene assumptions (e.g., known height). Existing learning based approaches circumvent this issue by reconstructing the 3D pose up to scale. However, there are many applications such as virtual telepresence, robotics, and augmented reality that require metric scale reconstruction. In this paper, we show that audio signals recorded along with an image, provide complementary information to reconstruct the metric 3D pose of the person. The key insight is that as the audio signals traverse across the 3D space, their interactions with the body provide metric information about the body's pose. Based on this insight, we introduce a time-invariant transfer function called pose kernel -- the impulse response of audio signals induced by the body pose. The main properties of the pose kernel are that (1) its envelope highly correlates with 3D pose, (2) the time response corresponds to arrival time, indicating the metric distance to the microphone, and (3) it is invariant to changes in the scene geometry configurations. Therefore, it is readily generalizable to unseen scenes. We design a multi-stage 3D CNN that fuses audio and visual signals and learns to reconstruct 3D pose in a metric scale. We show that our multi-modal method produces accurate metric reconstruction in real world scenes, which is not possible with state-of-the-art lifting approaches including parametric mesh regression and depth regression.

==> conclusion.tex <==
\section{Conclusion \label{sec:conc}}

This paper exploited the possibility of adding ultrasound audio as a new modality for metric scale 3D human pose estimation. By estimating a audio pose kernel, and encoding it to the physical space, we introduced a neural network pipeline that can accurately predict up to scale 3D human pose. We tested our algorithm on two unseen environments, and the results are promising, shading light towards potential application in smart home, AR/VR, human robot interaction, and beyond. We also proposed a new dataset DatasetName, calling for attentions from future researchers to this interesting audio-visual 3D pose estimation problem.

==> old_texts.tex <==

\clearpage

\section{Old texts}
\section{Dataset}
* We collected synchronized audio and vision data in 6 different environments across 6 different people.
* Data is recording using a Zoom F8n field recorder with commercial speakers and mics.
* Each person is asked to perform daily tasks in the environments while our audio and vision sensors are recording.
* In all environments, audio sensor and camera are registered to the same environment using colmap.
* The result is a dataset consisting of 5000 frames
\section{Implementation}
* We train using a batch size of xxx, and learning rate of xxx.
* Data is being trained on a server with 8xv100 GPUs for xx hours.
\section{Evaluation}
* We perform different kinds of test showing that our algorithm is working across different environments
* We compare with a base line where no audio sensor is used, and conducted a ablation study showing the performance gain with increased number of audio sensors



In this section, we will elaborate on how audio impulse response is related to geometry, and how we eventually encode audio responses into the 3D space for pose landmark likelihood estimation. We will start from a simple example illustrating how audio changes with respect to geometry, and then dive deep into the mathematics behind.

\textbf{Will sound change according to geometry (or pose)?}
Consider a simple example where a cubic object is placed in a room.
We use a speaker to shine a signal towards the object, and use a microphone to capture the signal bouncing off the object and room, as shown in figure \ref{fig:encoding_pose_kernel}.
We rotate the object around its center and plot the \textit{cross correlation} value between the received signal when (1) object is at pose $\theta$ ($R(\theta)$) and (2) object is at initial pose $\theta_0$ ($R(\theta_0)$)
We can see that cross correlation changes with different pose $\theta$.

\begin{figure}[hbt].
\centering
\vspace{-0.05in}
\includegraphics[width=\linewidth]{dummy.pdf}
\vspace{-0.25in}
\caption{(a) Simulation scenario, (b) Signal cross correlation value changes with respect to pose $\theta$}
\label{fig:encoding_pose_kernel} 
\vspace{-0.05in}
\end{figure}

This is because, different pose of the object creates different reflection profile (or echos) of the sound, and eventually leading to the variation of sound signal received by the microphone.


\textbf{Inferring geometry from sound:}
Now let us bring more maths to the problem. 
We first consider an open space without room echos.
Assume the speaker is placed at location $P_s$, and microphone is placed at location $P_m$.
Denote the transmitted sound from speaker as $s(t)$ and received sound captured from microphone as $r(t)$.
As we talked about in section 3.1, we can estimate an impulse response $k(t)$ caused by sound reflections through deconvolving $r(t)$ with $s(t)$.

As shown in figure \ref{fig:impulse}(a), there are a bunch of peaks in the impulse response $k(t)$. We use a Dirac delta function $\delta(t-t_i)$ to represent each peak at time $t = t_i$
Thus the impulse response can be represented as:
\begin{equation}
    k(t) = \sum_{i = 1} ^N A_i \cdot\delta(t - t_i)
\end{equation}
where $A_i$ is the amplitude of the peak, and $N$ is the total number of peaks.

\begin{figure}[hbt].
\centering
\vspace{-0.05in}
\includegraphics[width=\linewidth]{dummy.pdf}
\vspace{-0.25in}
\caption{(a) Impulse response illustration. (b) A peak in impulse response corresponds to a potential reflector on the eclipse.}
\label{fig:impulse} 
\vspace{-0.05in}
\end{figure}

For a given peak $A_i \delta(t-t_i)$ at time instance $t = t_i$, it actually corresponds to a reflection path of the audio signal. This is true because after convolution with original source signal $s(t)$, the result is a delayed and attenuated copy of original source signal $s(t)$, or in other words, creating echo $s^i(t)$ where
\begin{equation}
    s^i(t) = A_i \delta(t - t_i) * s(t) = A_i s(t - t_i)
\end{equation}

This means, each peak $A_i \delta(t-t_i)$ in the impulse response $k$, corresponds to a signal path with time of flight equals to $t_i$.
Then, basic physics tells us the distance between the microphone speaker pair and the reflector would be 
\begin{equation}
\label{equation:distance}
    d_{im} + d_{is} = t_i \cdot v
\end{equation}
where $v$ is the speed of sound, and $d_{im,s}$ are the distances between the $i^th$ reflector and the microphone, speaker.
This implies, the reflector is on an ecilipse trajectory with the speaker and mic at the 2 focuses, as shown in figure \ref{fig:impulse}(b).

Then let us consider the case where the reflector is inside a room.
By measuring in the scenario with and without person, we can get $2$ impulse responses $k(t)$ and $k_0(t)$, and a subtraction will give the human related impulse response $k_j(t)$ (measured at the $j^{th}$ speaker and microphone pair) as:
\begin{equation}
    k_j(t) = k(t) - k_0(t)
\end{equation}
Finally by applying the physics from equation \ref{equation:distance}, we connect this human related impulse response $k_j$ with human pose geometry.

\textbf{Spatial encoding of audio impulse response:}
We encode audio impulse response to 3D and creates an audio heatmap $W_j\in [0,1]^{D\times D\times D}$ in the physical frame (discretized into $D\times D\times D$), according to the audio-geometry math above.
One important thing to note, however, is that, unlike vision, the speaker and microphone that we use do not offer bearing information. Any point in the 3D space with the same distance to the speaker/mic pair will provide exactly the same time-of-flight, and thus contributes exactly the same to the audio impulse response.
To fully recover this omni-directional characteristic, we use a the following method for data encoding:

Assume the microphone is located at $P_{jm}(x_m,y_m,z_m)$, and speaker is located at $P_{jm}(x_s,y_s,z_s)$ in the global frame.
Then for any given point $P(x,y,z)$, the 3D heatmap value $W_j(x, y, z)$ would be:
\begin{equation}
    W_j(x, y, z) = k_j((d_{jm} + d_{js}) / v)
\end{equation}
where $k_j$ is the human related impulse response and $d_{jm,s}$ are the distances between point $P$ and the microphone, speaker location $P_{jm,s}$, i.e.,
\begin{align}
    d_{jm} &= ||(x_0,y_0,z_0)-(x_m,y_m,z_m)||_2 \\
    d_{js} &= ||(x_0,y_0,z_0)-(x_s,y_s,z_s)||_2
\end{align}


\textbf{Spatial encoding of vision data:}
Vision data is encoded similarly based on propagation model.
The major difference, is, however, vision ray is directional, but does not offer timing information.
We hope a fusion of audio and vision will provide us both bearing, and depth, and thus a 3D human pose.
Recall that for any given image, each pixel on the 2D image corresponds to one ray in the 3D space, obtained from camera intrinsic matrix.
We use OpenPose \cite{openpose} to get 2D joint location for 15 joints on the human body.
These 15 2D joint location are then projected into the 3D space to form 15 signal ray.
Any given point on each of these rays is a possible 3D joint location.
For the purpose of data smoothing, we use a Gaussian representation of the ray to create a 3D heatmap.

Finally, after encoding audio and vision data to the 3D space, we directly regress joint heatmap from this 3D space.



%(talk about how $k_j(t)$ can be translated to distance based on equation, and relate it with $\mathbf{X}$ above.
%==> what is missing in 3.1 is the spatial relationship between speaker and mic and how that are related to 3D arbitrary point. This needs to be explained thoroughly with equations)
%(you can talk about toy example to show geometric insight.)
\subsection{Objective function and Implementation}
%Talk about overall objective function that you use and design of neural network. 
We used 3D CNN as building blocks to directly regress pose from the $D\times D\times D$ heatmaps for audio and vision.
A multi stage 3D CNN pipeline is proposed, and short cuts are introduced to prevent potential gradient vanishing.
We also adopted a max pooling layer for audio signals after audio feature extracting, so that neural network will not memorize the audio sensor sequence for the sake of best generalizability.
We estimate the joint heatmaps for each of the joints, and a mean square loss is reported at the end of each stage.
The final loss is the sum of all losses for each stage:
\begin{equation}
    L = \sum_{i = 1}^N L_i
\end{equation}


\subsection{Overview}
Single view human pose lifting is the problem of estimating 3D human pose from a 2D image, defined by the following equation, where $X$ is the 3D human pose, and $I$ is the 2D image:
\begin{equation}
\label{equ:problem_orig}
    X = f(I)
\end{equation}
Due to the lack of depth information, an infinitive number of poses will match with the 2D image. In other words, this is an ill defined problem.

Sound, given its relatively slow speed of propagation, offers a unique opportunity of distance estimation.
Imagine we have a couple of speakers and microphones in the environment.
By emitting sound from speakers and collecting signals reflected off human body at the microphone side, we can estimate the time-of-flight of sound, which can translate to depth measurement (for each body joint).
While theoretically plausible, there are, of course a lot of challenges given the dispersive nature of sound, causing heavy multipaths, especially in indoor environments.

This paper focus on tackling all the challenges and including a new modality, audio $A$, into the pipeline of 3D pose estimation, mathematically denoted as:
\begin{equation}
\label{equ:problem_our}
    X = f(I, A)
\end{equation}
More specifically, to extract as much spatial information as we can from audio, we deployed multiple audio sensors (speakers and microphones) around the environment, giving us $k$ different audio measurements $A_1, A_2, ..., A_k$ for each pose:
\begin{equation}
\label{equ:problem_our}
    X = f(I, A_1, A_2, ..., A_k)
\end{equation}
A signal processing pipeline $h(\cdot)$ is proposed to effectively cope with the indoor audio multipath, and encode 1D audio data to 3D heatmap space.
Similarly, vision information is also encoded to 3D space through a function $g(\cdot)$:
\begin{equation}
\label{equ:problem_our_specific}
    X = f(g(I), h(A_1), h(A_2), ..., h(A_k))
\end{equation}
Finally a 3D CNN is trained on the audio and vision 3D heatmaps to regress human joint locations.

In the rest of this section, we will first give an experimental study showing the feasibility of the idea from signal's perspective.
Then we will elaborate on each component of the pipeline, especially how we design $f$, $g$, and $h$.
Let us first start with feasibility study.


\subsection{Feasibility study: can audio infer geometry?}
\textbf{Acoustic simulation result:}


\textbf{Real world toy example:}
Now let us move to the real world experiment of human pose estimation.
We ask the person to stand still in the same location, while doing different poses.
Similarly, we also record the \textit{cross correlation} value $xcorr$ between two human poses $P_1$ and $P_2$.
We ask the person to do a fixed list of poses, for multiple times.
Table \ref{table:toy} shows the result.
It is evident that if for the same pose, the xcorr value is high, while for different poses, xcorr value is low.
This implies the promise of using audio as a method for pose estimation.

\subsection{How to infer geometry: signal processing background}
%Introduce RIR
%Introduce subtraction of RIR
%Note that we need to send a sequence of sample to infer channel impulse response. Signal frequency selection



%\subsection{Audio signal preprocessing and encoding}

%\section{Background and Measurement}

However, most of the times, the echos are merged with the original sound signal, making it difficult to interpret.
%Figure \ref{fig:signal}(a) shows a simple scenario where there are 3 reflectors in the environment and figure \ref{fig:signal}(b) shows the raw received signal and the source signal being played.
%It is evident that echo signals cannot be easily observed from the received signal.
%\begin{figure}[hbt].
%\centering
%\vspace{-0.05in}
%\includegraphics[width=\linewidth]{dummy.pdf}
%\vspace{-0.25in}
%\caption{}
%\label{fig:signal} 
%\vspace{-0.05in}
%\end{figure}
To extract the reflection profile (or more technically the time domain impulse response $h$), we perform a deconvolution between the receiver signal $R$ and the source signal $S$ \cite{}.
\begin{equation}
    h = R *^{-1} S
\end{equation}
In an ideal case where there is no multipath reflection, each object in the environment will correspond to one Dirac delta function in the impulse response.
%In the example case, we can observe 3 peaks each corresponds to one reflecting object (as shown in figure \ref{fig:signal}(c)).
Assume the speaker and microphone are co-located and synchronized, the location of the peaks exactly represent the time-of-flight.

\textbf{Estimating distance in rich multipath indoor environment}:
Then let us move to a more realistic scenario.
In a typical indoor room environment, where there are a lot of echos, instead of getting a bunch of clear Delta functions in the impulse response, what we get is a complex time domain function with a lot of peaks merged together.
Figure \ref{fig:rir}(a) shows a typical room impulse response.
Each of these peak corresponds to a reflecting surface in the environment, e.g., walls, ceilings, furniture, etc.
Given the massive number of reflecting surfaces and their complex reflecting property, understanding geometry from this complex signal would be prohibitive if not impossible.

However, recall that our goal is to reconstruct human pose, so we are not exactly interested in those room reflections.
What we really need to extract are those human related reflections.
Now, imagine we have 2 time domain impulses, one with person and one without person, as shown in figure \ref{fig:rir}(a) and (b).
If we align them properly and perform a subtraction, the static environmental reflections will be cancelled out, and the result is human related reflections, as shown in figure \ref{fig:rir}(c).
Different peaks in figure \ref{fig:rir}(c) ideally corresponds to reflections from different body parts, and this serves as the physics foundation of the paper.
With the increasing popularity of always-on mics in today's smart voice assistants, it is easy to perform a scan of the room, and get an accurate empty room impulse response.
Building on this, we designed our system.

\begin{figure}[hbt].
\centering
\vspace{-0.05in}
\includegraphics[width=\linewidth]{dummy.pdf}
\vspace{-0.25in}
\caption{}
\label{fig:rir} 
\vspace{-0.05in}
\end{figure}

\subsection{Data encoding}
To make our model as general possible,
we adopt a physics based approach to model how signal propagates.
This is because, both audio and vision follows the physics way of propagation.
We try to directly regress the 3D pose from the 3D space based on signal propagation physics.
Let us start with audio data encoding.
\\
\textbf{Audio data encoding:}
Recall that we already have the one dimensional impulse response (after subtracting empty room response), the next task would be connecting this with 3D geometry.
Note that the speaker and microphone that we use do not offer bearing information, any point in the 3D space with the same distance to the speaker/mic pair will provide exactly the same response.
This implies the polar coordinate system based 3D encoding method.
Assume the sensor’s location is denoted as $(x_0,y_0,z_0)$ in the global frame.
Then for any given location $P(x,y,z)$, the response equals to $RIR(|(x_0,y_0,z_0)-(x,y,z)|)$\\
\textbf{Vision data encoding:}
Vision data is encoded similarly based on propagation model.
The major difference, is, however, vision ray is directional, but does not offer timing information.
We hope a fusion of audio and vision will provide us both bearing, and depth, and thus a 3D human pose.
Recall that for any given imagre, each pixel on the 2D image corresponds to one ray in the 3D space.
We use OpenPose \cite{} to get 2D joint location for 15 joints on the human body.
These 15 2D joint location are then projected into the 3D space to form 15 signal ray.
Any given point on each of these rays is a possible 3D joint location.
For the purpose of data smoothing, we use a Gaussian representation of the ray to create a 3D heatmap.\\
\textbf{Groundtruth encoding}
Similar with Convolutional Pose Machine \cite{}, for joint labels, we also use a 3D gaussian distribution located at the groundtruth joint location in the 3D space.
* Finally a 3D CNN is trained to regress the vision rays and audio RIR heatmap to every joint location
\subsection{Network architecture}
* We use 3D convolution layer as the basic building block of our network.
* Input has 4 audio heatmap channels and 15 vision Ray heatmap channels.
* Output is 15 channels of joint heatmaps
* Considering the high dimensionality of our data, we have multiple blocks of network.
* Each block output is compared with groundtruth to obtain a L2 loss.
* We added shortcuts to avoid the potential gradient vanishing problem
* We train the network for minimizing the sum of all L2 losses.




% \begin{table*}[hbt]
% \begin{center}
%  \renewcommand{\arraystretch}{0.8}
% \begin{tabular}{L{2cm}| C{2cm}| C{2cm}| C{2cm}| C{3cm}| C{3cm}}
%  \hline
%   & \multicolumn{3}{c}{Ours} & \multicolumn{2}{|c}{Baseline}\\
%   \hline
%  Scenario & 4 pairs audio + vision &  2 pairs audio + vision & vision only & Frankmocap + average height & Simplify + average height \\
%   \hline
%  Avg. 3D joint loc. err& 11.35cm&11.77cm& xxxcm &19.01cm & xxxcm\\
%  \hline
%   Avg. human center loc. err& 9.14cm&9.53cm& xxxcm &18.84cm & xxxcm\\
%  \hline
%   PCK& &&&&\\
%   t = 10 cm & 0.476 & 0.449 & xxx & 0.873 & xxx \\
%   t = 20 cm & 0.843 & 0.834 & xxx & 0.638 & xxx \\
%   t = 30 cm & 0.966 & 0.963 & xxx & 0.992 & xxx \\
%   t = 40 cm & 0.991 & 0.990 & xxx & 0.970 & xxx \\
%  \hline
%  PJE (cm) & &&&&\\
% Head &8.89&10.43&xx&17.99&xx\\
% L Hand&12.14&12.07&xx&18.93&xx\\
% L Elbow&11.39&11.30&xx&19.11&xx\\
% L Shoulder&9.90&10.81&xx&18.71&xx\\
% Neck&8.35&9.95&xx&18.45&xx\\
% R Shoulder&9.04&10.39&xx&18.24&xx\\
% R Elbow&10.32&11.14&xx&18.28&xx\\
% R Hand&11.72&12.97&xx&18.18&xx\\
% L Foot&15.29&13.77&xx&20.81&xx\\
% L Knee&13.75&12.43&xx&19.71&xx\\
% L Hip&11.23&10.90&xx&19.17&xx\\
% C Hip&10.78&11.27&xx&18.89&xx\\
% R Hip&11.20&11.68&xx&19.00&xx\\
% R Knee&12.85&13.12&xx&19.27&xx\\
% R Foot&13.39&14.39&xx&20.43&xx\\
%  \hline
 
% \end{tabular}
%  \renewcommand{\arraystretch}{1}
% \end{center}
% \caption{PoseKernelLift result on environment A (kid). PoseKernelLifter is significantly better than vision only solutions due to the ambiguity of scale for vision only methods.}
% \label{tab:main_result_a}
% \end{table*}


% \begin{table*}[hbt]
% \begin{center}
%  \renewcommand{\arraystretch}{0.8}
% \begin{tabular}{L{2cm}| C{2cm}| C{2cm}| C{2cm}| C{3cm}| C{3cm}}
%  \hline
%   & \multicolumn{3}{c}{Ours} & \multicolumn{2}{|c}{Baseline}\\
%   \hline
%  Scenario & 4 pairs audio + vision &  2 pairs audio + vision & vision only & Frankmocap + average height & Simplify + average height \\
%   \hline
%  Avg. 3D joint loc. err& 11.35cm&11.77cm& xxxcm &19.01cm & xxxcm\\
%  \hline
%   Avg. human center loc. err& 9.14cm&9.53cm& xxxcm &18.84cm & xxxcm\\
%  \hline
%   PCK& &&&&\\
%   t = 10 cm & 0.476 & 0.449 & xxx & 0.873 & xxx \\
%   t = 20 cm & 0.843 & 0.834 & xxx & 0.638 & xxx \\
%   t = 30 cm & 0.966 & 0.963 & xxx & 0.992 & xxx \\
%   t = 40 cm & 0.991 & 0.990 & xxx & 0.970 & xxx \\
%  \hline
% PJE (cm) & &&&&\\
% Head &8.89&10.43&xx&17.99&xx\\
% L Hand&12.14&12.07&xx&18.93&xx\\
% L Elbow&11.39&11.30&xx&19.11&xx\\
% L Shoulder&9.90&10.81&xx&18.71&xx\\
% Neck&8.35&9.95&xx&18.45&xx\\
% R Shoulder&9.04&10.39&xx&18.24&xx\\
% R Elbow&10.32&11.14&xx&18.28&xx\\
% R Hand&11.72&12.97&xx&18.18&xx\\
% L Foot&15.29&13.77&xx&20.81&xx\\
% L Knee&13.75&12.43&xx&19.71&xx\\
% L Hip&11.23&10.90&xx&19.17&xx\\
% C Hip&10.78&11.27&xx&18.89&xx\\
% R Hip&11.20&11.68&xx&19.00&xx\\
% R Knee&12.85&13.12&xx&19.27&xx\\
% R Foot&13.39&14.39&xx&20.43&xx\\
%  \hline
 
% \end{tabular}
%  \renewcommand{\arraystretch}{1}
% \end{center}
% \caption{PoseKernelLift result on environment B (adult). PoseKernelLifter produces similar results with vision-only methods, due to vision-only network memorizing average human height.}
% \label{tab:main_result_b}
% \end{table*}

